Towards Disentangled Speech Representations

The careful construction of audio representations has become a dominant feature in the design of approaches to many speech tasks. Increasingly, such approaches have emphasized "disentanglement", where a representation contains only parts of the speech signal relevant to transcription while discarding irrelevant information. In this paper, we construct a representation learning task based on joint modeling of ASR and TTS, and seek to learn a representation of audio that disentangles that part of the speech signal that is relevant to transcription from that part which is not. We present empirical evidence that successfully finding such a representation is tied to the randomness inherent in training. We then make the observation that these desired, disentangled solutions to the optimization problem possess unique statistical properties. Finally, we show that enforcing these properties during training improves WER by 24.5% relative on average for our joint modeling task. These observations motivate a novel approach to learning effective audio representations.

==> modeling_improvements.tex <==
\section{Modeling Improvements \label{sec:modeling}}


\subsection{Base Architecture: Cascaded Encoders}

As first presented in \cite{arun21cascade}, the baseline model we consider in this work is a \emph{Cascaded Encoders} model, as shown in Figure \ref{fig:cascade}. In this model, the 1st-pass system consists of a causal encoder followed by an RNN-T decoder (prediction network + joint layer). In the second pass, the additional non-causal layers take in both left and right context of the 1st-pass encoder outputs, and are fed to the same decoder. A single RNN-T decoder is shared between the 1st and 2nd-passes for better long-form performance, and smaller model size and on-device benefits. Improvements to this model will be discussed below.

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.35]{figs/cascaded_encoder.png}
  \caption{A block diagram of the Cascaded Encoders model.}
   \label{fig:cascade}
   \vspace{-0.1in}
\end{figure}


% The work in \cite{arun21cascade,bo21system} explored using conformer layers \cite{gulati2020conformer} for the causal and non-causal encoders, and LSTM layers for the prediction network. In this work, we explore reducing computation \st{on device} with an embedding decoder. In addition, we explore training the model with a HAT factorization, so that a neural LM can be integrated during decoding. All three components are discussed below.

\subsection{Embedding Prediction Network}   \label{sec:emb-decoder}
The broad success of neural networks in machine learning has brought customized hardware, both in servers and in consumer devices, that can process these networks efficiently. However, these devices are less efficient at processing auto-regressive or recurrent models. Therefore, in this work we explore making the auto-regressive prediction + joint layers in Figure \ref{fig:cascade} as small and efficient as possible. Specifically, we replace the LSTM prediction network with an embedding lookup table, and share the parameters of the embedding table with the softmax layer. Below we briefly describe the embedding network, shown in Figure \ref{fig:embedding}, and refer the reader to \cite{Rami21} for more details. 


% User-perceived latency is measured as the response time of the server after a user finishes a query. Running a second-pass beam search requires a minimal delay in output to not impact user-perceived latency, which motivates using a small decoder.  In addition, improvements with hardware accelerators have made it possible to run models even faster on-device. However, these accelerators have a small memory footprint and operate best when the entire network can fit in-memory, as the latency cost moving parameters from CPU to TPU is high. 



%While there have been lots of work in the literature using limited context decoders
%Although limited context modeling for decoders has been explored in several studies, most suffer from a quality degradation compared to an LSTM decoder \cite{Variani20,ghodsi2020rnn,zhang2021tiny}. In this work, we explore two changes to the embedding decoder to address previous performance degradation issues. A diagram of the embedding prediction network is shown in Figure \ref{fig:embedding}.


\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.275]{figs/embedding_decoder.png}
  \caption{Block diagram of Embedding Prediction Network.}
   \label{fig:embedding}
   \vspace{-0.1in}
\end{figure}

With the embedding network, given the 5 previous non-blank predictions from the model, which we denote as $Y_{prev} = \{y_{u-5}, \ldots, y_{u-1}\}$, we look up the embedding of each of these outputs, denoted as $\{e_5, \ldots, e_1\}$. The embedding table is of size $|V| \times d_e$, where $|V|$ is the vocabulary size (i.e. wordpieces) and $d_e$ is the embedding dimension. Thus each $e_i$ is of size $d_e$.
For each position in the label history $Y_{prev}$, we create a random, constant position vector $PV=\{p_5, \ldots, p_1\}$ and take a dot product of each $p_i$ with embedding $e_i$, and average this, giving output $\bar a_1$.  The intuition for the $PV$ is that it allows for embeddings to be attended over in proportion to how relevant they are to their respective positions. Motivated by \cite{Vaswani17}, the operation from embeddings $\{e_5, \ldots, e_1\}$ to embedding averaging $\bar a_1$ is replicated across multiple heads $H$, which improves performance at the cost of a small parameter increase. Each head shares the same embedding table, but has unique $PVs$. The embeddings across each head are also averaged together to get the final embedding vector $\bar{a}_{final}= \frac{1}{H} \sum_i^H \bar a_i$. 

Neural networks can model a more complex function with additional linear-layer + non-linearity. Since the embedding layer is a simple lookup table, we improved modeling expressiveness, again at the cost of a small parameter increase, by passing the final averaged embedding vector, $\bar{a}_{final}$, through a projection layer and Swish non-linearity, to get output $r$. 

Finally, the joint layer, as shown in Figure \ref{fig:cascade}, takes the output of the prediction network, $r$, and encoder network, $ce_t$ (causal) or $nce_t$ (non-causal), projects this to dimension $d_h$ and then passes it to a softmax layer, which is of size $d_h \times (|V| + 1)$, with the extra output for the blank token. By setting $d_e=d_h$, we share the weights between the embedding and softmax matrices for all non-blank tokens, to further reduce decoder size. This is similar to weight tying used in language modeling \cite{inan2016tying}. 

\subsection{HAT Factorization}

An E2E model directly estimates the posterior of word sequence, $y$, conditioned on the acoustic features, $x$, i.e.,  $p(y|x)$. A common way to integrate an E2E model with an external LM that estimates $p_{LM}(y)$ is to perform shallow fusion (Eq \ref{eq:shallow_fusion}).

%, as shown in Equation~\ref{eq:shallow_fusion}:
\begin{equation}
\centering
y^* = \arg \max_y \left[\log p(y|x) + \lambda_1 \log p_{LM}(y)\right]
\label{eq:shallow_fusion}
\end{equation}
Here, $\lambda_1$ is the weight given to the LM. Since E2E models tend to be over-confident in their posterior estimates, weighting the two terms becomes difficult and can often lead to high deletions \cite{Chorowski17}.  To address this issue, Hybrid Autoregressive Transducer (HAT) proposes a way to factor out an internal LM score, $p_{ILM}(y)$, so that the likelihood score from the E2E model, $p(x|y)$, can be approximated by Equation \ref{eq:ilm}:
\begin{equation}
\centering
\log p(x|y) \approx \log p(y|x) - \log p_{ILM}(y)
\label{eq:ilm}
\end{equation}

The HAT factorization makes it mathematically more stable to then integrate an E2E model with an external LM, without needing additional coverage penalties:
\begin{equation}
\centering
y^* = \arg \max_y \left[\log p(y|x) - \lambda_2 \log p_{ILM}(y) + \lambda_1 \log p_{LM}(y) \right]
\label{eq:hat}
\end{equation}
Here, $\lambda_1$ and $\lambda_2$ are the weights on the LM and ILM, respectively. We train the cascaded encoder with a HAT factorization to allow for better integration with a neural LM and biasing LM.  %discussed in the next section.

\subsection{Neural Language Model} \label{sec:lm}
Our large-scale text-data corpus has $\sim$100 billion utterances, and spans domains of Maps, News, Google Play, Web and YouTube. In contrast, the supervised audio-text pairs used to train the E2E model is much smaller (300 million) and includes domains such as Search, Dictation, YouTube and Telephony~\cite{Arun19}. Challenges related to domain-mismatch and data scale make it difficult to train neural LMs using both these datasets. 

N-gram LMs attempt to handle the scale and domain-mismatch of the data by training a separate model on each individual domain and then performing a Bayesian interpolation~\cite{Allauzen11} to optimize performance on a target domain of interest. Maximum entropy training, used to train such models, incorporates various optimization strategies to speed up model training, resulting in training on billions of examples taking less than one day \cite{Biadsy17}. Furthermore, to address domain-mismatch, \cite{Biadsy20} proposes fine-tuning just on the supervised set after pre-training on all the data. 
In this work, we address these challenges by simply mixing the LM data and transcripts form the supervised training data with equal probability. 
% In this paper, we do not look to address the data scale issue of neural LMs, and thus our training takes more than one week. To handle the domain mismatch, we mix the LM data and supervised training data with equal probability.

%Because the training of neural LMs is a non-convex optimization problem requiring small minibatches, training across all domains cannot be as easily parallelized\ARUN{This sentence seems out of place in this paragraph.}. Note that while mixture-of-expert neural LMs \cite{Irie2018} is one possible approach to handle the domain-mismatch issue, it often increases model size and is, therefore, not considered in this work. 



Because of the on-device latency limitations, we explore using a conformer LM to \emph{rescore} hypotheses from the 2nd-pass non-causal decoder. One of the benefits of transformer/conformer LMs is that there is no self-recurrence in the model. This means that model outputs can be computed for multiple inputs in parallel. This is particularly effective in rescoring when the inputs to the LM is known ahead of time. Transformer LMs have shown promising results in the literature \cite{Devlin2018,Dai2019,Keskar2019}. In this work, given our promising results with conformer encoder \cite{gulati2020conformer}, we explore using a unidirectional conformer LM, where we only attend on previous tokens.

\subsection{Biasing \label{biasing_section}}

Contextual biasing~\cite{Petar15} increases the likelihood of the ASR system recognizing contextually-relevant phrases, such as names from the user's contact list. The typical approach for biasing is to interpolate scores from the E2E model $\log p(y|x)$ and a contextual LM $\log p_{C}(y)$, represented by a weighted finite-state transducer (FST), via shallow fusion \emph{during} the beam search~\cite{Ding19}. We explore how biasing performance is improved with HAT, as shown in Equation \ref{eq:biasing}. When contextual biasing is applied during beam search to the causal and non-causal decoders, the weight of the neural LM $\lambda_1=0$. Note that $\lambda_1\neq0$ during rescoring with the neural LM, and the contextual LM is reapplied so as to not undo the effects of biasing when applied during beam search. $\beta$ is the cost on the contextual LM.

\begin{equation}
\begin{split}
y^* = \arg \max_y [&\log p(y|x) - \lambda_2 \log p_{ILM}(y)\ + \\ 
& \lambda_1 \log p_{LM}(y) + \beta \log p_{C}(y) ]
\label{eq:biasing}
\vspace{-0.2in}
\end{split}
\end{equation}

%In this paper we explore different approaches of improving the performance of E2E contextual biasing for specific domains. The contextual biasing models are represented as grapheme-based weighted, deterministic, finite state acceptors (WDFSA) and are applied to the E2E model's wordpieces. We specifically explore if using the HAT internal-LM cost helps to improve performance when integrating WDFSA. 

%using a grapheme-to-wordpiece speller.

% Expand on the contextual biasing models themselves
%\subsubsection{Contextual Models}
%In E2E contextual biasing \cite{Ding19}, we distribute the weights of each biasing phrase on each arc along its path in the WDFSA. Additionally we add failure arcs to the start at each state to undo the bias for any mismatches. This is necessary since we eagerly apply the bias before the whole biasing phrase matches and limits overly biasing towards phrase prefixes. Additionally we limit the adverse effects of applying the contextual biasing models to anti-context utterances by prepending the weighted portion of the biasing phrase with an unweighted prefix phrase. We use commonly used prefix phrases in the desired context, for example a song is usually prefixed with "play" and a contact name is prefixed with "call" or "text".

%\subsubsection{Grapheme-to-Wordpiece Speller}
%The grapheme-to-wordpiece speller utilizes a pre-constructed mapping between wordpieces and graphemes. This allows the decoder to match the wordpiece outputs from the E2E model to the grapheme-based contextual biasing models. This has the benefits of the contextual biasing model being able to consider any wordpiece sequence for a word.

% Eager biasing

%\subsubsection{Shallow Fusion}
%For first method we apply the contextual (biasing) LMs on the E2E model directly using shallow fusion. The contextual biasing models are applied at each wordpiece output of the E2E model. This has been found previously to show improvement over just apply biasing at the word boundaries \cite{Ding19}. In this approach, the bias is applied on the total score and is not bounded. This means that although the bias is from a contextual biasing LM, it could be over-bias and overwrite the AM score portion of total score.

%\subsubsection{On-the-fly Lattice LM Rescoring}
%To address the undesired effect of over-biasing and overwriting the AM score by the contextual biasing, in the second method we only apply the contextual biasing models on the LM score. This is made possible given the HAT factorization of the ILM. In this paper the LM rescoring is applied to the ILM during the 1st-pass decoding and on the external LM during the 2nd-pass.

%The LM rescoring is done by applying the contextual biasing models on the wordpiece lattice via on-the-fly lattice rescoring.  The on-the-fly lattice rescoring is applied to the LM score and a minimum score of zero is set for the LM score by applying a softplus to the combined weight. This limits the impact of contextual biasing to the LM as opposed to the total score. When multiple paths have the same interpolated LM score from biasing, this allows the AM score to be used to determine the best path.

%\PMR{qnlethe@, it wasn't immediately obvious to me that LM rescoring happens to both the ILM and external LM. Maybe call it out in the text.}

%In addition to the on-the-fly lattice LM rescoring, a contextual model for shallow fusion is used as well. In this case, the shallow fusion score is only used during the beam search to affect the pruning. 

%\PMR{qnlethe@, should we cite the Amazon paper for the latter?}

\subsection{Latency \label{prefecth_section}}

To decode the cascade model in the streaming system, we run the 1st-pass \textit{causal decoder} and the 2nd-pass \textit{non-causal decoder} in parallel. The causal decoder is faster while the non-causal decoder is more accurate. Hence, to reduce latency, the causal decoder is responsible for emitting the partial recognition results \cite{yu21fastemit} and endpointing \cite{li2020towards} quickly. Once the endpointing decision is declared, the system then closes the microphone and sends the final recognition result decoded thus far by the non-causal decoder to the server. %This is another reason why having a small embedding decoder is beneficial.
%Therefore, the cascade model could preserve the quick endpointing by the causal decoder as well as the accurate final result by the non-causal decoder.

%\subsubsection{Prefetch in cascade model} %\label{prefecth_section}

%In addition to quick endpointing.
An additional way to reduce latency is to fetch results even before the final recognition is ready, which is referred to as prefetching~\cite{chang2020prefetch}. If the partial result matches the final recognition result, the response fetched for the partial result can be delivered to the user instantly and save the execution latency that typically happens after recognition is completed.

%A comparison of different prefetch mechanisms in the E2E system is presented in \cite{chang2020prefetch}.

In the cascade model, partial results and final results are emitted by separate decoders. The mismatch can increase prefetch miss, which makes the prefetched results unusable, thereby increasing latency. To reduce the mismatch, we propose to prefetch results based on the combination of both decoders, referred to as \textit{hybrid prefetching}. To merge the prefetch decision from the causal and non-casual decoders, the system first generates prefetch candidates from both decoders independently and then discards the results if they are stale. A prefetch candidate is marked as stale if the top hypotheses is a substring of the latest valid prefetch. For example, ``navigate" is a stale result as compared to ``navigate to home" so that prefetch is not overridden by the late hypothesis. In the hybrid scenario, the quicker prefetch by the causal decoder would dominate while more accurate prefetch by the non-causal decoder could still revert incorrect prefetching for corner cases. 
%\begin{table}[h!]
%    \centering
%    \begin{tabular}{|c|c|c|} \hline
%    Model & median latency & 90th latency\\ \hline
%    prefetch by casusal decoder & 120 & 380 \\ \hline
%    hybrid prefetch & 110 & 250  \\ \hline
%    \end{tabular}
%    \caption{Prefetch latency on Search}
%    \vspace{-0.2in}
%    \label{tab:prefetch}
%\end{table}

